Sublinear-time Reductions for Big Data Computing

With the rapid popularization of big data, the dichotomy between tractable and intractable problems in big data computing has been shifted. Sublinear time, rather than polynomial time, has recently been regarded as the new standard of tractability in big data computing. This change brings the demand for new methodologies in computational complexity theory in the context of big data. Based on the prior work for sublinear-time complexity classes \cite{DBLP:journals/tcs/GaoLML20}, this paper focuses on sublinear-time reductions specialized for problems in big data computing. First, the pseudo-sublinear-time reduction is proposed and the complexity classes \Pproblem and \PsT are proved to be closed under it. To establish \PsT-intractability for certain problems in \Pproblem, we find the first problem in $\Pproblem \setminus \PsT$. Using the pseudo-sublinear-time reduction, we prove that the nearest edge query is in \PsT but the algebraic equation root problem is not. Then, the pseudo-polylog-time reduction is introduced and the complexity class \PsPL is proved to be closed under it. The \PsT-completeness under it is regarded as an evidence that some problems can not be solved in polylogarithmic time after a polynomial-time preprocessing, unless \PsT = \PsPL. We prove that all \PsT-complete problems are also \Pproblem-complete, which gives a further direction for identifying \PsT-complete problems.

==> pseudo-log-time.tex <==
\section{Pseudo-log-time Reduction}\label{sec:ps-red}

In this section, we introduce the notion of pseudo-log-time reduction.

\begin{definition}\label{def:ps-red}
	\emph{
		A decision problem $\CP_1$ is \textit{pseudo-log-time reducible} to a decision problem $\CP_2$, denoted as $\CP_1 \le^{\tt PsL}_m \CP_2$, if there exists a triple $\langle f_1(\cdot), f_2(\cdot), g(\cdot, \cdot)\rangle$,
		where $f_1(\cdot)$ and $f_2(\cdot)$ are \NC computable functions and $g(\cdot, \cdot)$ is a $\PPL^1$ computable function, such that for any pair of strings $\langle D, P\rangle$ it holds that
		\[\langle D, P\rangle \in \CP_1 \Leftrightarrow \langle f_1(D), g(f_2(D), P) \rangle \in \CP_2.\]
	}
\end{definition}

%Since \DLOG is the first level of \PPL hierarchy identified in \cite{DBLP:journals/tcs/GaoLML20}, $g(\cdot, \cdot)$ is required to be computable in \DLOG.
%For optimization problems, we need not only the functions converting the data part and problem part of $\CP_1$ to corresponding part of $\CP_2$, but also a \DLOG computable function $h(\cdot, \cdot)$ mapping the solution of $\CP_2$ back into the solution of $\CP_1$.
%We now verify the properties of $\le^{\tt PsL}_m$.
In pseudo-log-time reduction, we 

\begin{theorem}
	If $\CP_1 \le^{\tt PsL}_m \CP_2$ and $\CP_2 \le^{\tt PsL}_m \CP_3$, then also $\CP_1 \le^{\tt PsL}_m \CP_3$.
\end{theorem}

\begin{proof}
	From $\CP_1 \le^{\tt PsL}_m \CP_2$ and $\CP_2 \le^{\tt PsL}_m \CP_3$, it is known that there exist four \NC computable functions $f_1(\cdot)$, $f_2(\cdot)$, $f'_1(\cdot)$, and $f'_2(\cdot)$, and two \DLOG computable functions $g(\cdot, \cdot)$ and $g'(\cdot, \cdot)$ such that for all $D_1$, $P_1 \in \CP_1$ defined on $D_1$, $D_2$, and $P_2 \in \CP_2$ defined on $D_2$ it holds that
	\[\langle D_1, P_1 \rangle \in \CP_1 \Leftrightarrow \langle f_1(D_1), g(f_2(D_1), P_1) \rangle \in \CP_2,\]
	\[\langle D_2, P_2 \rangle \in \CP_2 \Leftrightarrow \langle f'_1(D_2), g'(f'_2(D_2), P_2) \rangle \in \CP_3.\]
	
	To show $\CP_1 \le^{\tt PsL}_m \CP_3$, we define two \NC computable functions $f''_1(\cdot)$, $f''_2(\cdot)$ and a \DLOG computable function $g''(\cdot, \cdot)$ as required in Definition \ref{def:ps-red}.
	Now, let $f''_1(x) = f'_1(f_1(x))$, $f''_2(x) = \llcorner|f_2(x)|\lrcorner\#f_2(x)\#f'_2(f_1(x))$ and $g''(x, y) = g'(p , g(q, y))$ if $x = \llcorner|p|\lrcorner\#p\#q$, where \# is a special symbol that is not used anywhere else.
	%计算串的二进制长度属于L，L属于NC
	Then we have
	\begin{equation*}
		\begin{aligned}
			\langle D_1, P_1 \rangle \in \CP_1 &\Leftrightarrow \langle f_1(D_1), g(f_2(D_1), P_1)\rangle \in \CP_2\\
			&\Leftrightarrow \langle f'_1(f_1(D_1)), g'(f'_2(f_1(D_1)), g(f_2(D_1), P_1)) \rangle \in \CP_3\\
			&\Leftrightarrow \langle f''_1(D_1), g''(\llcorner|f_2(D_1)|\lrcorner\#f_2(D_1)\#f'_2(f_1(D_1)), P_1) \rangle \in \CP_3\\
			&\Leftrightarrow \langle f''_1(D_1), g''(f''_2(D_1), P_1) \rangle \in \CP_3
		\end{aligned}
	\end{equation*}
	It is easy to verify that $f''_1(\cdot)$ and $f''_2(\cdot)$ are in \NC and $g''(\cdot, \cdot)$ is in \DLOG.
	\qed
\end{proof}

\begin{theorem}\label{thm:ps-close}
	For each $i \ge 1$, the complexity class  $\PsPL^i$ is closed under $\le^{\tt PsL}_m$.
\end{theorem}

\begin{proof}
	From $\CP_1 \le^{\tt PsL}_m \CP_2$, we know that there exist two \NC computable functions $f_1(\cdot)$, $f_2(\cdot)$, and a \DLOG computable function $g(\cdot,\cdot)$ such that for all $D_1$ and $P_1 \in \CP_1$ defined on $D_1$ it holds that
	\[\langle D_1, P_1\rangle \in \CP_1 \Leftrightarrow \langle f_1(D_1), g(f_2(D_1), P_1)\rangle \in \CP_2.\]
	Furthermore, since $\CP_2 \in \PsPL$, there exists a \PTIME preprocessing function $\Pre_2(\cdot)$ such that for all $D_2$ and $P_2 \in \CP_2$ defined on $D_2$: $P_2(\Pre_2(D_2)) = P_2(D_2)$, and $P_2(\Pre_2(D_2))$ can be solved by a \RATM $M_2$ in $O(\log^{c_2}{|D_2|})$ for some $c_2 \ge 1$.
	Therefore, for all $D_1$ and $P_1\in \CP_1$ defined on $D_1$ we have,
	\[P_1(D_1) = g(f_2(D_1), P_1)(f_1(D_1)) = g(f_2(D_1), P_1)({\rm\Pi_2}(f_1(D_1))).\]
	
	To show $\CP_1 \in \PsPL$, we claim that there exist a \PTIME preprocessing function ${\rm \Pi_1}(\cdot)$ for $\CP_1$ such that $P_1(D_1) = P_1({\rm\Pi_1}(D_1))$ and a \RATM for $P_1({\rm\Pi}_1(D_1))$ running in polylogarithmic time as required in Definition \ref{def:pspl}.
	First, let ${\rm\Pi_1}(x) = \llcorner|f_2(x)|\lrcorner\#f_2(x)\#{\rm\Pi_2}(f_1(x))$, where $\#$ is a special symbol that is not used anywhere else.
	Then we construct a \RATM $M_1$ by appending a pre-procedure to $M_2$.
	More concretely, with input ${\rm\Pi_1}(D_1)$ and $P_1$, $M_1$ first copies $\llcorner|f_2(x)|\lrcorner$ to one of its work tapes and computes the index of the second $\#$, which equals to $|f_2(x)| + |\llcorner|f_2(x)|\lrcorner| + 1$.
	Then $M_1$ generates $g(f_2(D_1), P_1)$ according to the information between the two \#s.
	Finally, $M_1$ simulates the computation of $M_2$ with input ${\rm\Pi}_2(f_1(D_1))$ behind the second \# and $g(f_2(D_1), P_1)$, then outputs the result returned by $M_2$.
	
	Since ${\rm\Pi_2}(\cdot)$ is in \PTIME, $f_1(\cdot)$ and $f_2(\cdot)$ are in \NC, and the length of a string is logarithmic time computable ${\rm\Pi_1}(\cdot)$ is obviously in \PTIME.
	Notice that computing the index of the second \# requires $t_I = O(\log{|f_2(D_1)|})$ time and $g(\cdot, \cdot)$ is computable in time $O(\log{|f_2(D_1)|})$.
	Therefore, the total running time of $M_1$ is bounded by $t_I + t_g + t_{M_2} = O(\log{|f_2(D_1)|} + \log^{c_2}{|f_1(D_1)|}) = O(\log^{c_1}{|D_1|})$ where $c_1 = \max\{1, c_2\}$.
	Thus, $\CP_1 \in \PsPL$.
	\qed
\end{proof}


Since reductions define difficulty orders of problems in a complexity class, the complete problem is regarded as the hardest one.
We define \PsPL-complete problems as follows.
\begin{definition}
	\emph{
		A problem $\CP$ is {\rm \PsPL}-hard under pseudo-logtime reduction if $\CP' \le^{\tt PsL}_m \CP$ for all $\CP' \in \PsPL$.
		A problem is {\rm \PsPL}-complete under pseudo-logtime reduction if $\CP$ is \PsPL-hard and $\CP \in \PsPL$.
	}
\end{definition}

We give a specified range of possible complete problems for \PsPL, by relating them to the following well-known \Pproblem-complete problem.
Given a graph $G$, a depth-first search(DFS) traverses $G$ in a particular order by picking an unvisited vertex $v$ from the neighbors of the most recently visited vertex $u$ to search, and backtracks to the vertex from where it came when a vertex $u$ has explored all possible ways to search further.\smallskip


\noindent Ordered Depth-First Search (ODFS):\vspace{-1ex}
\begin{itemize}
	\item[$\circ$]{\bf Given:} A graph $G = (V, E)$ with fixed adjacent lists, fixed starting vertex $s$, and vertices $u$ and $v$.
	\item[$\circ$]{\bf Problem:} Does vertex $u$ get visited before vertex $v$ in the DFS traversal of $G$ starting from $s$? 
\end{itemize}

\begin{theorem}{\rm \cite{DBLP:journals/ipl/Reif85}}\label{odfs:pcomplete}
	{\rm ODFS} is {\rm \Pproblem}-complete under \NC reduction.
\end{theorem}

\begin{theorem}
	Given a problem $\CP$, if $\CP$ is {\rm \PsPL}-complete, then $\CP$ is {\rm \Pproblem}-complete.
\end{theorem}

\begin{proof}
	It is easy to see that ${\rm ODFS}$ is in $\PsPL$.
	Since $\CP$ is \PsPL-complete, ${\rm ODFS} \le^{\tt PsL}_m \CP$.
	That is, there exist two \NC computable functions $f_1(\cdot)$, $f_2(\cdot)$ and a \DLOG computable function $g(\cdot,\cdot)$ such that for all $G, s, (u, v) \in {\rm ODFS}$ it holds that
	\[\langle G\circ s, (u, v)\rangle \in {\rm ODFS} \Leftrightarrow \langle f_1(G\circ s), g(f_2(G\circ s), (u, v))\rangle \in \CP.\]
	As stated in Theorem \ref{odfs:pcomplete}, ODFS is \Pproblem-complete under \NC reduction.
	For any problem $L \in \Pproblem$, there is a \NC computable function $h(\cdot)$ such that
	\[x \in L \Leftrightarrow h(x) \in {\rm ODFS}.\]
	Recall that the input of ODFS consists of a graph $G$, a starting point $s$, and two vertices $u, v$.
	It is easy to modify the output format of $h(x)$ to $\llcorner|G\circ s|\lrcorner\#G\circ s\#(u,v)$ in \NC.
	Now let $f'_1(x) = f_1(y)$ and $g'(x) = g(f_2(y), z)$, if $x = \llcorner|y|\lrcorner\#y\#z$.
	Consequently, it follows that
	\[x \in L \Leftrightarrow \langle h(x).G\circ s, h(x).(u, v)\rangle \in {\rm ODFS} \Leftrightarrow \langle f'_1(h(x)), g'( h(x))\rangle \in \CP.\]
	Let $h'(x) = f'_1(h(x))\circ g'(h(x))$ to concentrate two parts of $\CP$ we can see that $L$ is \NC reducible to $\CP$.
	Moreover, $\PsPL \subseteq \Pproblem$.
	Therefore, $\CP$ is \Pproblem-complete.
	\qed
\end{proof}

In the breakthrough work of dynamic DFS on undirected graphs~\cite{DBLP:conf/soda/BaswanaCC016}, Baswana \etal defined a nearest edge query between a subtree and an ancestor-descendant path in the procedure of rerooting a DFS tree, which was used in almost all subsequent work.
Chen et al. showed that this query could be solved by running a range successor query~\cite{DBLP:conf/swat/ChenDWZZ18}.
We refine the procedure as a pseudo-logtime reduction. 
The definitions of these two problems are given as follows.\smallskip

\noindent Nearest Edge Query (NEQ):\vspace{-1ex}
\begin{itemize}
	\item[$\circ$]{\bf Given:} A DFS tree $T$ of graph $G$, the endpoints $x, y$ of an ancestor-descendant path, the root $w$ of a subtree $T(w)$ such that $par(w) \in path(x, y)$.
	\item[$\circ$]{\bf Problem:} Find the edge $e$ that is incident nearest to $x$ among all edges between $T(w)$ and $path(x, y)$.
\end{itemize}

\noindent Range Successor Query (RSQ):\vspace{-1ex}
\begin{itemize}
	\item[$\circ$]{\bf Given:} A set of $d$-dimensional points $S$, a query rectangle $Q = {\rm \Pi}^d_{i = 1}[a_i, b_i]$.
	\item[$\circ$]{\bf Problem:} Find the point $p$ with smallest $x$-coordinate among all points that are in the rectangle $Q$.
\end{itemize}

\begin{theorem}{\rm \cite{DBLP:conf/swat/ChenDWZZ18}}
	${\rm NEQ} \le_m^{\tt PsL} {\rm RSQ}$.
\end{theorem}

\begin{proof}
	Given a graph $G = (V, E)$ and a DFS tree $T$ of $G$, define $f_1:E \to S$ as follows, where $S$ is a set of $2$-dimensional points.
	Denote the preorder traversal sequence of $T$ by $\rho$, note that every subtree of $T$ can be represented by a continuous interval of $\rho$.
	Let $\rho(v)$ denote the index of vertex $v$ in this sequence that is if $v$ is the $i$-th element in $\rho$, then $\rho(v) = i$.
	For each edge $(u, v) \in E$, $f_1((u, v)) = (\rho(u), \rho(v))$.
	That is for each edge $(u, v)$, a point $(\rho(u), \rho(v))$ is added into $S$.
	Notice that for each point $p \in S$, there exists exactly one edge $(u, v)$ associated with $p$.
	Next we state the information provided by $f_2(\cdot)$.
	For each vertex $v$, let $\gamma(v) = \max_{w \in T(v)}\rho(w)$, \ie, the maximum index of vertices in $T(v)$.
	Thus, define $f_2(v)$ as $\rho(v)\#\gamma(v)$ for each $v \in V$.
	
	Then, to answer an arbitrary query instance $T(w), p(x, y)$, let $g$ be the function mapping $w, x, y$ to a rectangles ${\rm\Omega} = [\rho(x),\rho(w) - 1]\times[\rho(w), \gamma(w)]$.
	Finally, given a point $p \in S$ as the final result of RSQ, let $h(\cdot, \cdot)$ be reverse function of $f_1(\cdot)$, \ie, it returns the edge of $G$ corresponding to $p$.
	It is easily to verify that the edge corresponding to the point with minimum x-coordinate is the edge nearest to $x$ among all edges between $T(w)$ and $path(x, y)$ \cite{DBLP:conf/swat/ChenDWZZ18}.
	
	The preorder traversal sequence of $T$ can be obtained by performing a DFS on it, which can be done in \NC as stated in \cite{smith1986parallel}.
	Therefore, both $f_1(\cdot)$ and $f_2(\cdot)$ are \NC computable.
	As for $g(\cdot, \cdot)$ and $h(\cdot, \cdot)$, with the mapping provided by $f_2(\cdot)$, both of them can be computed in logarithmic time.
	\qed
\end{proof}

There is numerous work showing that RSQ belongs to \PsPL \cite{DBLP:conf/swat/NekrichN12}.
Hence, with the fact that pseudo-logtime reduction is compatible with \PsPL, the following corollary is obtained.

\begin{corollary}
	${\rm NEQ} \in $ {\rm \PsPL}.
\end{corollary}

